SyntheX: Scaling Up Learning-based X-ray Image Analysis Through In Silico Experiments

Artificial intelligence (AI) now enables automated interpretation of medical images for clinical use. However, AI's potential use for interventional images (versus those involved in triage or diagnosis), such as for guidance during surgery, remains largely untapped. This is because surgical AI systems are currently trained using post hoc analysis of data collected during live surgeries, which has fundamental and practical limitations, including ethical considerations, expense, scalability, data integrity, and a lack of ground truth. Here, we demonstrate that creating realistic simulated images from human models is a viable alternative and complement to large-scale in situ data collection. We show that training AI image analysis models on realistically synthesized data, combined with contemporary domain generalization or adaptation techniques, results in models that on real data perform comparably to models trained on a precisely matched real data training set. Because synthetic generation of training data from human-based models scales easily, we find that our model transfer paradigm for X-ray image analysis, which we refer to as SyntheX, can even outperform real data-trained models due to the effectiveness of training on a larger dataset. We demonstrate the potential of SyntheX on three clinical tasks: Hip image analysis, surgical robotic tool detection, and COVID-19 lung lesion segmentation. SyntheX provides an opportunity to drastically accelerate the conception, design, and evaluation of intelligent systems for X-ray-based medicine. In addition, simulated image environments provide the opportunity to test novel instrumentation, design complementary surgical approaches, and envision novel techniques that improve outcomes, save time, or mitigate human error, freed from the ethical and practical considerations of live human data collection.

==> excess_text.tex <==
but fall short of offering significant clinical advantages over a human surgeon because the data basis inhibits more innovative endeavours.


While robotic platforms and the benefits of introducing them are well documented, e.\,g.,  for gastrointestinal~\cite{TODO an axel krieger paper} or ocular micro-surgery~\cite{TODO A gelbach paper}, none of these systems can be considered truly autonomous, which posits another challenge: Robotic actions, clinical decisions, and thus, the overall dynamics of the procedure are still shaped by the human surgeon. 
Therefore, considering all aforementioned challenges, for autonomous surgical systems to reach their full potential, taking advantage of advanced computer vision and robotic manipulation, will require sources of data independent from human operators.

==> old_text.tex <==
Text we deleted from the full manuscript because it seemed duplicate
%We confront the primary challenge facing this paradigm: the frustrating inability of learning-based systems to generalize beyond a single, compact domain. Here, the compact domain encompasses images from a specific X-ray simulation software, called DeepDRR. Like any simulator, DeepDRR produces image with some shared characteristics that differ from real X-rays, including overall image appearance, noise patterns and correlation, contrast, and resolution, which constrain the high-dimensional image domain. While the shape and extent of this domain is unknown, it can be approximated with a sufficiently large sample of simulated X-rays, which are easy to generate at scale. Likewise, the domain of real X-ray images (collected intra-operatively) can be approximated with a dataset, although real images are more difficult to collect and annotate. A \emph{domain gap} exists because these two classes of images are distinct, although they contain the same semantic content, causing a significant performance drop when algorithms are trained in simulation and evaluated in the real. This \emph{Sim2Real} drop has been observed among multiple medical imaging tasks~\cite{mahmood2018deep, gu2020extended, bier2019learning}.


%Over the past decade, the general computer vision community has developed two major approaches to mitigate domain gap problem: Domain Randomization~(DR) and Domain Adaptation~(DA). The first, which originated in general robotics~\cite{tobin2017domain}, relies on random changes in the simulator's characteristics during training. This produces a training set with many separate domains, in the hopes that the target domain lives inside their convex hull. The second method, DA, attempts to mitigate the domain gap's detrimental effect using an adversarial domain classifier, which discourages domain-specific features~\cite{ganin2015unsupervised}. DA is especially well-suited for the \emph{Sim2Real} because it allows for unlabeled data in the target domain. The widely used CycleGAN algorithm~\cite{zhu2017unpaired}, for example, uses DA to transform images between domains without correspondence labels of images in each domain.

%In the context of medical imaging, DR and DA have \emph{Sim2Real} improvements, but the interaction of these methods with the characteristics of specific simulators has yet to be quantified. These choices directly affect the ability of any vision-based surgical agent to generalize across the \emph{Sim2Real} gap. Small changes to the simulator properties may cause large performance drops in the real. The mystery surrounding these effects in autonomous X-ray image analysis imposes an upper limit on the frontier of AI algorithms in clinical practice.

old text that we reworked

% \section{Introduction}
% Learning based methods are redefining the state-of-the-art possibilities across a large variety of difficult problems, including robot visual servoing, scene understanding and image interpretation. However, the generality and real world performance of these methods hinge on the representativeness/quality of the dataset that was used to train them. Creating large representative datasets is clearly challenging because of many reasons including representative data sampling, data archiving and labeling, and in medicine even more due to the requirement of domain knowledge and privacy concerns. Therefore, simulation paradigms have become a major research thrust in general CV already~\cite{shah2018airsim, qiu2016unrealcv, muller2018sim4cv}. Frameworks exist for animation and motion planning~\cite{ju2013data, kutbi2019learning}, scene understanding~\cite{papon2015semantic}, semantic segmentation~\cite{ros2016synthia}, object pose estimation~\cite{chen2019pose}, object recognition~\cite{hejrati2014analysis}, human gesture estimation~\cite{hoffmann2019learning}, etc.

% In medicine, similar approaches exist for ultrasound imaging~\cite{mattausch2018realistic} and MRI~\cite{liu2016fast} but primarily X-ray based applications. Because of the invertible physics of Computed Tomography~(CT), X-ray images can be simulated from 3D CT scanning, which is called Digitally Reconstructed Radiograph~(DRR). Since pre-operative CT scan is generally available and easy to annotate, it is feasible to generate large scale labeled dataset via DRR simulation. Thus, researchers have attempted to apply learning-based methods on radiography data fusion challenges, such as segmentation~\cite{li2016automatic}, object or landmark detection~\cite{bier2019learning}, 2D/3D registration~\cite{gu2020extended, miao2017dilated}, 3D reconstruction~\cite{shen2019patient}, task-aware imaging~\cite{zaech2019learning}, etc.

% However, the issue in these scenarios is that performance of learning-based methods in general can only be guaranteed on compact domains, which are composed of data derived from simulators. Such compact domains usually share different properties compared to the real world data domains such as image appearance, noise patterns, etc. Therefore, a significant \textit{Sim2Real} performance drop has been observed among multiple medical imaging tasks caused by this domain gap. Mahmood et al. proposed a joint deep convolutional neural network-conditional random field (CNN-CRF) framework for depth estimation on colonoscopic images. Their method achieved a relative error of 0.183 in \textit{Sim2Sim}, but the \textit{Sim2Real} performance dropped to 0.242~\cite{mahmood2018deep}. Gu et al. proposed a sequential CNN-based method for extending 2D/3D registration capture range. The \textit{Sim2Sim} mean registration error was 1.58 mm/0.12 degrees, but the \textit{Sim2Real} error was 39.4 mm/6.95 degrees in translation and rotation, respectively~\cite{gu2020extended}. Bier et al. proposed a view-invariant pelvis anatomical landmark detection network and achieved average \textit{Sim2Sim} $l_2$ distance error of $5.6\pm4.5$ mm. However, the error increased to 15-20 mm when testing on real cadaveric X-ray images~\cite{bier2019learning}. Methods for \textit{Sim2Real} transfer are highly sought to bridge this generalization gap.

% Domain Randomization~(DR) is firstly proposed to address this generalization gap in robotics simulation~\cite{tobin2017domain}. DR training introduces drastic data augmentation in order to sample a large variation of data appearances. Significant improvements have been observed with DR training on the tasks of object detection~\cite{tremblay2018training}, robot grasping~\cite{tobin2018domain}, autonomous driving~\cite{pan2017virtual}, etc. Recent works have shown that the \textit{Sim2Real} performance in medical imaging tasks can also be boosted with DR. Toth et al. applied DR on the task of 3D/2D cardiac model-to-X-ray registration. The mean registration error on clinical data was 18.45~mm/2.26~degrees with No DR and 0.75~mm/1.06~degrees with combined DR~\cite{toth2019training}. Grimm et al used DR for fully automatic X-ray to CT registration~\cite{grimm2020pose}. They found that networks trained with DR on simulated X-rays can better transfer to real X-rays.
% % \cg{TODO: describe what has not been done in literature for DR comparison and the importance of our study}

% Domain Adaptation~(DA) refers to learning a discriminative classifier in the presence of a shift between source and target domain~\cite{ganin2015unsupervised}. DA is useful for \textit{Sim2Real} in the sense that mappings between domains can still be learned when target domain data are fully unlabeled or very few samples are labeled. CycleGAN is one popular DA approach for learning image style transfer from source to target domain~\cite{zhu2017unpaired}. It has been investigated in X-ray angiography to generate more training data while conserving the anatomical integrity of arteries and realistic X-ray patterns~\cite{tmenova2019cyclegan}. Adversarial Discriminative Domain Adaptation~(ADDA) is another typical DA approach~\cite{tzeng2017adversarial}. It trains a discriminator which predicts domain labels using features encoded from source and target domain images. Haq et al. applied ADDA for cell segmentation~\cite{haq2020adversarial}, which shows superior \textit{Sim2Real} performance compared to baseline models.

% Image-based registration is one of the key procedures to integrate intra-operative images with pre-operative planning, navigate surgical tools without the need of manual annotations or additional hardwares.  Deep learning in medical imaging suffers the problem of acquiring real training data and annotations. Some imaging modalities, such as fluoroscopy X-ray images, can be simulated from CT scans.  However, deep networks trained on simulation images will overfit to the simulation domain, which leads to large performance drop when testing on real images. It is thus important to bridge the generalization gap between simulation and real images.

% \section{Methodology}

% We present the details of generating simulation images from different DRR generators using pose estimation from real X-ray image annotations. We then talk about the domain randomization and adaptation techniques we used for this ablation study.
% \section{Data availability}
% Our previous study has published an accurately annotated dataset of 366 real hip fluoroscopic images taken from six cadaveric specimens~\cite{grupp2020automatic}. Metallic BBs were injected to the pelvic anatomies. lower torso CT scan of each specimen was acquired after BB injection. 3D and 2D BB locations were manually annotated in each CT and X-ray image. Therefore, the pelvis pose with respect to the C-arm frame was estimated by solving the PnP problem for each X-ray image.

% 6 anatomical structures and 14 landmarks were annotated in each CT scan. The anatomical structures include left and right hemipelvis, vertebrae, upper sacrum, left and right femurs. 3D anatomical landmarks consist of left and right: anterior superior iliac spine~(ASIS), center of femoral head~(FH), superior pubic symphysis~(SPS), inferior pubic symphysis~(IPS), medial obturator foramen~(MOF), inferior obturator foramen~(IOF), and the greater sciatic notch~(GSN). These landmarks are useful in identifying the anterior pelvic plane~(APP) and initializing the pelvis 2D/3D registration~\cite{gao2020tmrb, nikou2000description}. 3D segmentations and landmarks were projected to 2D using the pelvis pose estimation of each X-ray image. The 2D segmentations and landmarks serve as labels in  multi-task learning.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.5\textwidth]{fig/landmark_geom.png}
%     \caption{Pose geometry and landmark annotation. }
%     \label{fig:landmark_geom}
% \end{figure}

% In order to setup a precisely controlled study to benchmark \textit{Sim2Real} performance, we used the CT scans and pose estimations to generate DRR simulation images, which have the exact same projection views of the paired real images. Three different DRR simulators were selected. They are na\"ive DRR, xreg DRR\footnote{https://github.com/rg2/xreg}~\cite{grupp2019pose} and DeepDRR~\cite{unberath2018deepdrr}. na\"ive DRR only considers mano-energetic source, single material attenuation coefficient, and neglects image corruption, e.g., due to noise or scattering. xreg DRR performs a linear thresholding of the CT Hounsfield Units~(HU) recordings to differentiate materials between air and anatomy. DeepDRR simulates a full spectrum of the X-ray photon energy, and relies on machine learning for material decomposition and scatter estimation. Both xreg DRR and DeepDRR inject noise during simulation. Fig.~\ref{fig:drr_simulations} presents an example comparison of different image appearance using DRR generators and real X-ray image.

% To further demonstrate the performance of multi-task learning with simulation images, we selected 20 CT scans from the New Mexico Decedent Image Database~\cite{newmexico}. We annotated 3D anatomical segmentations and landmarks and then generated 500 DeepDRR images with randomly sampled projection geometries for each CT scan, resulting in a total of 10,000 simulation images. Segmentation and landmark labels were propagated from 3D to 2D for each image. All images and labels for both datasets were downsampled to three resolution levels: $180\times180$, $360\times360$ and $480\times480$.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.40\textwidth]{fig/DRR_simulations.png}
%     \caption{Example DRR simulations. Left to right: Naive DRR, Xreg DRR, DeepDRR and the corresponding real X-ray image. }
%     \label{fig:drr_simulations}
% \end{figure}

% \subsection{Network Architecture}
% Our network architecture is using the approach described by~\cite{grupp2020automatic, gao2019localizing}. It extends the 6-level U-Net~\cite{ronneberger2015u} with concurrent segmentation and landmark localization branches. The network loss composes of an averaged dice score over each class for segmentation~($L_{seg}$) and an averaged normalized cross-correlation~(NCC) between groundtruth heatmap and the corresponding estimate for landmark localization~($L_{ld}$).

% \subsection{Domain Randomization}

% \section{Experiments and Results}



% \begin{table}[h!]
% \footnotesize
% \centering
% \caption {Segmentation DICE score over 6-fold validation. We limit cycleGAN here to naive DRRs.}
% \begin{tabular}{ |c|c|c|c|c| }
% \hline
%  & No DR & Regular DR & Strong DR & ADDA\\
% \hline
% NaiveDRR &  $0.67 \pm 0.25$ & $0.69\pm0.27$ & $0.66\pm0.28$ & $0.74\pm 0.25$\\
% \hline
% XregDRR & $0.65\pm0.26$  & $0.73\pm0.26$ & $0.78\pm0.21$ & $0.76\pm0.24$\\
% \hline
% DeepDRR & $0.68\pm0.25$ & $0.76\pm0.24$ & $0.78\pm0.22$ & $0.77\pm0.24$\\
% \hline
% cycleGAN & $0.70\pm0.26$  & $0.77\pm0.22$ & $0.77\pm0.22$ & $0.74\pm0.25$\\
% %\hline
% %DeepDRR-cycleGAN & $0.71\pm0.26$ & $0.80\pm0.19$ & $0.79\pm0.21$ & $0.77\pm0.24$\\
% \hline
% Real   & $0.74\pm0.24$  & $0.81\pm0.20$ & $0.82\pm0.20$ & $--$\\
% \hline
% \end{tabular}
% \label{table-seg}
% \end{table}




% \yh{Here I made some visualization figures for individual landmark errors (total 14) and for individual segmentation labels (total 6), summarizing 8x experiments. Some landmark detection results, for example, Land14, seems not sexy to me because of the large std among all experiments (including real2real). Next \todo{\textcolor{red}{  Following Cong's style to make a plot for all dice performance?}}  }

% \begin{figure}[h!]

%     \includegraphics[width = \textwidth, left]{fig/Landmark1_plot.png}
%     \includegraphics[width = \textwidth, left]{fig/Landmark14_plot.png}
%     \caption{Performance visualization for individual landmark detection. On the left side, individual landmark annotations are visualized from 3D slicer. On the right side, Real2Real performance are reported with \textcolor{orange}{yellow markers}. Experiments with better performance (lower error) are reported with \textcolor{green}{green markers}. Similarly, those with reduced performance (larger error) are reported with \textcolor{red}{red markers}.    }
%     \label{fig:landmark_individual}
% \end{figure}

% \begin{figure}[h!]

%     \includegraphics[width = \textwidth, left]{fig/Segmentation1_plot.png}
%     \includegraphics[width = \textwidth, left]{fig/Segmentation6_plot.png}
%     \caption{Performance visualization for segmentation across all six labels. On the left side, each of labels (Left Hemipelvis, Right Hemipelvis, Vetebrae, Upper Sacrum, Left Femur, and Right Femur) are visualized from 3D slicer. On the right side, Real2Real performance are reported with \textcolor{orange}{yellow markers}. Experiments with better performance (greater dice) are reported with \textcolor{green}{green markers}. Similarly, those with reduced performance (lower dice) are reported with \textcolor{red}{red markers}.}
%     \label{fig:dice_individual}
% \end{figure}

% that's all folks

some commented out table
% Segmentation score with higher order digits
% \begin{table*}[t!]
% \caption {Segmentation Dice Score}
% \label{table-dice}
% \centering
% \begin{tabular}{ |c|c|c|c|c|c|c| }
% \hline
%  & \multicolumn{2}{|c|}{180x180} & \multicolumn{2}{|c|}{360x360} & \multicolumn{2}{|c|}{480x480}\\
% \cline{2-7}
%  & regular DR & strong DR & regular DR & strong DR & regular DR & strong DR\\
% \hline
%     RealXray & $0.7750\pm0.2348$  & $0.7840\pm0.2142$ & $0.7828\pm0.2320$ & $0.7585\pm0.2484$ & $0.7394\pm0.2658$ & $0.7511\pm0.2645$\\
% \hline
%     Realistic  & $0.7298\pm0.2400$ & $0.7869\pm0.2108$ & $0.7510\pm0.2407$ & $0.7602\pm0.2497$ & $0.7204\pm0.2558$ & $0.6999\pm0.2788$ \\
% \hline
%     Naive & $0.6892\pm0.2558$ & $0.6799\pm0.2782$ & $0.6866\pm0.2657$ & $0.5719\pm0.3092$ & $0.6533\pm0.2779$ & $0.5780\pm0.3050$\\
% \hline
%     Heuristic & $0.6694\pm0.2728$ & $0.7368\pm0.2491$ & $0.6833\pm0.2645$ & $0.6816\pm0.2858$ & $0.6551\pm0.2767$ & $0.6681\pm0.2975$\\
% \hline
%     Realistic-CycleGAN & $0.7779\pm0.2171$ & $0.7779\pm0.2195$ & $0.7602\pm0.2477$ & $0.7334\pm0.2673$  & $0.7411\pm0.2554$ & $0.6877\pm0.2906$\\
% \hline
%     Naive-CycleGAN & $0.7843\pm0.1976$ & $0.7498\pm0.2296$ & $0.7392\pm0.2543$ & $0.7357\pm0.2580$ & $0.7263\pm0.2537$ & $0.6729\pm0.2917$\\
% \hline
%     Realistic-ADDA & $0.7672\pm0.2235$ & $0.7537\pm0.2310$ & $0.7255\pm0.2922$ & $0.3845\pm0.4178$ & $16.42\pm37.61$ & $9.24\pm17.53$\\
% \hline
%     Naive-ADDA & $0.4907\pm0.4045$ & $0.6777\pm0.2660$ & $0.6931\pm0.2974$ & $0.6620\pm0.2649$ & $16.62\pm40.12$ & $22.88\pm41.53$\\
% \hline
%     Realistic-NM & $5.91\pm8.43$ & $**\pm**$ & $6.80\pm9.53$ & $6.29\pm6.29$ & $8.12\pm19.35$ & $5.99\pm12.19$\\
% \hline
%     Realistic-CycleGAN-NM & $6.79\pm9.70$ & $6.87\pm9.58$ & $6.87\pm13.19$ & $6.59\pm7.25$ & $6.43\pm13.67$ & $5.52\pm4.85$\\
% \hline
% \end{tabular}
% \vspace{0.5em}
% \end{table*}

